A New Complexity Metric for Nonconvex Rank-one Generalized Matrix Completion

In this work, we develop a new complexity metric for an important class of low-rank matrix optimization problems in both symmetric and asymmetric cases, where the metric aims to quantify the complexity of the nonconvex optimization landscape of each problem and the success of local search methods in solving the problem. The existing literature has focused on two complexity bounds. The RIP constant is commonly used to characterize the complexity of matrix sensing problems. On the other hand, the incoherence and the sampling rate are used when analyzing matrix completion problems. The proposed complexity metric has the potential to generalize these two notions and also applies to a much larger class of problems. To mathematically study the properties of this metric, we focus on the rank-$1$ generalized matrix completion problem and illustrate the usefulness of the new complexity metric on three types of instances, namely, instances with the RIP condition, instances obeying the Bernoulli sampling model, and a synthetic example. We show that the complexity metric exhibits a consistent behavior in the three cases, even when other existing conditions fail to provide theoretical guarantees. These observations provide a strong implication that the new complexity metric has the potential to generalize various conditions of optimization complexity proposed for different applications. Furthermore, we establish theoretical results to provide sufficient and necessary conditions for the existence of spurious solutions in terms of the proposed complexity metric. This contrasts with the RIP and incoherence conditions that fail to provide any necessary condition.

==> deleted_part.tex <==
By suitably generalizing the definitions of $\mathbb{D}_\alpha(C,u^*)$ and $\cD$, the results in Theorem \ref{thm:rip-1} can be extended to the general problem \eqref{eqn:obj-bm} in the rank-$1$ case with a slightly weaker bound. 
In this work, we provide one possible generalization. 
For the problem \eqref{eqn:obj-bm}, each instance is defined by the loss function $f(\cdot;\cdot)$ and the ground truth $M^*$, which we denote as $(f,M^*)$. We assume that the loss function satisfies
% 
\begin{align}\label{eqn:normalization-3}
f(M^*;M^*) &= \min_{K\in\mathbb{R}^{n\times n}} {f}(K;{M}^*),\\
\nonumber&\hspace{6em}\forall M^*\in\R^{n\times n}\quad \st \quad M^*\succeq0,~ \rank(M^*)=1. 
\end{align}
% 
In the special case when $f(\cdot;\cdot)$ is the weighted $\ell_2$-loss function in \eqref{eqn:gmc}, the above condition implies that $C_{ij}\geq 0$ for all $i,j\in[n]$. Similar to the normalization constraint $C\in\Sn_{+,1}$, we consider any objective function $f(\cdot;M^*)$ with the property that
% 
\begin{align}\label{eqn:normalize-1} 
{\sum}_{i,j\in[n]} \left[f(M^* + E_{ij}; M^*) - f(M^*;M^*) \right] = 1, 
\end{align}
% 
where $E_{ij}$ is defined in \eqref{eqn:normalize}. For the normalization constraint $u^*\in\Snn_1$, we consider any global truth with the property that
% 
\begin{align}\label{eqn:normalization-2}
{\sum}_{i\in[n]} \sqrt{M^*_{ii}} = 1.
\end{align}
% 
The set of degenerate instances is given by
% 
\begin{align*}
    \cD := \bigg\{ &(f, M^*) ~\bigg|~f(\cdot;\cdot) \text{ and } M^* \text{ satisfy \eqref{eqn:normalization-3}- \eqref{eqn:normalization-2}},\\
    &\exists M\neq M^*\quad \st~ f(M;M^*) = f(M^*;M^*) , M^*\succeq0,\rank(M^*)=1 \bigg\}.
\end{align*}
% 
The ``entry-wise $\ell_1$-norm'' between two arbitrary functions $h^1(\cdot)$ and $h^2(\cdot)$ with the domain $\R^{n\times n}$ is defined as the restricted $\ell_\infty$-Lipschitz constant of $h^1-h^2$. Namely, we define $\|h^1-h^2\|_1$ to be
% 
\begin{align*}
     \|h^1-h^2\|_1 := \sup_{K,L\in\R^{n\times n}} &\frac{\left| \left(h^1(K) - h^2(K) \right) - \left(h^1(L) - h^2(L) \right) \right|}{\max_{i,j\in[n]} (K_{ij} - L_{ij})^2}\\
     \st \quad &K\neq L,\quad \rank(K-L) \leq 2.
\end{align*}
% 
For every constant $\alpha\in[0,1]$, the distance between two instances $(f,M^*)$ and $(\tilde{f},\tilde{M}^*)$ is defined as
% 
\begin{align*}
    &\dist_\alpha\left[ (f,M^*), (\tilde{f},\tilde{M}^*) \right] := \alpha\|f(\cdot;M^*) - \tilde{f}(\cdot;\tilde{M}^*)\|_1 + (1-\alpha)\|u^* - \tilde{u}^*\|_1,
    % &\hspace{5em} + \alpha \\
    % &+,
\end{align*}
% 
where $u^*,\tilde{u}^*\in\Rn$ satisfy $u^*(u^*)^T=M^*$ and $\tilde{u}^*(\tilde{u}^*)^T=\tilde{M}^*$. Finally, the complexity metric is given by
% 
\begin{align*}
    \mathbb{D}_\alpha(f,M^*) := \left[\inf_{(\tilde{f},\tilde{M}^*)\in\cD} \dist_\alpha\left[ (f,M^*), (\tilde{f},\tilde{M}^*) \right]\right]^{-1}.
\end{align*}
% 
We note that the definitions of $\cD$ and $\mathbb{D}_\alpha(f,M^*)$ are consistent with those of instance \eqref{eqn:gmc}. The following theorem provides an upper bound on the complexity metric of any instance satisfying the RIP$_{2,2}$ condition.
% 
\begin{theorem}\label{thm:rip-gen}
Let $\alpha\in[0,1]$ and $\delta\in[0,1)$ be two constants. Suppose that the function $f(\cdot;M^*)$ satisfies the $\delta$-RIP$_{2,2}$ condition and the normalization constraint \eqref{eqn:normalize-1}. Then, it holds that
% 
\[ \mathbb{D}_\alpha(f,M^*) \leq \frac{n^2(1+\delta)}{\alpha(1-\delta)}
% ,\quad \forall (\tilde{f},\tilde{M}^*) \in \cD. 
\]
% 
\end{theorem}
% 
\begin{proof}
We fix the instance $(f,M^*)$ and assume that $(\tilde{f},\tilde{M}^*)\in\cD$. Suppose that the matrix $M \neq \tilde{M}^*$ satisfies
% 
\[ {\sum}_{i\in[n]} \sqrt{M_{ii}} = 1,\quad \tilde{f}(M;\tilde{M}^*) = \tilde{f}(\tilde{M}^*;\tilde{M}^*). \]
% 
We first consider the case when $M \neq M^*$. In this case, we can estimate that
% 
\begin{align}\label{eqn:rip-general-1}
    &\|f(\cdot;M^*) - \tilde{f}(\cdot;\tilde{M}^*)\|_1\\
    \nonumber&\hspace{3em}\geq \frac{\left| \left[ f(M;M^*) - \tilde{f}(M;\tilde{M}^*) \right] - \left[ f(M^*;M^*) - \tilde{f}(M^*;\tilde{M}^*) \right] \right|}{\max_{i,j\in[n]} (M_{ij} - M_{ij}^*) ^2}\\
    \nonumber&\hspace{3em}= \frac{\left| \left[ f(M;M^*) - f(M^*;M^*) \right] + \left[ \tilde{f}(M^*;\tilde{M}^*) - \tilde{f}(M;\tilde{M}^*) \right] \right|}{\max_{i,j\in[n]} (M_{ij} - M_{ij}^*) ^2}\\
    \nonumber&\hspace{3em}= \frac{\left| \left[ f(M;M^*) - f(M^*;M^*) \right] + \left[ \tilde{f}(M^*;\tilde{M}^*) - \tilde{f}(\tilde{M}^*;\tilde{M}^*) \right] \right|}{\max_{i,j\in[n]} (M_{ij} - M_{ij}^*) ^2}\\
    \nonumber&\hspace{3em}\geq \frac{f(M;M^*) - f(M^*;M^*)}{\max_{i,j\in[n]} (M_{ij} - M_{ij}^*) ^2} \geq \frac{(c_1/2)\cdot \|M-M^*\|_F^2}{\max_{i,j\in[n]} (M_{ij} - M_{ij}^*) ^2} \geq \frac{c_1}{2},
\end{align}
% 
where $c_1$ is the constant in the RIP condition of $f(\cdot;M^*)$. The second inequality is due to
% 
\[ f(M;M^*) - f(M^*;M^*) \geq 0,\quad \tilde{f}(M^*;\tilde{M}^*) - \tilde{f}(\tilde{M}^*;\tilde{M}^*) \geq 0. \]
% 
The second last inequality follows from the global optimality of $M^*$ and the second inequality after inequality (12) in \cite{zhang2021general}, namely,
% 
\[ f(M;M^*) \geq f(M^*;M^*) + \frac{c_1}{2} \| M - M^*\|_F^2,\quad \forall M\in\R^{n\times n},~ \rank(M) \leq 1. \]
% 
Now, we provide a lower bound on $c_1$. Using the normalization constraint \eqref{eqn:normalize-1} and the stationarity of $M^*$, it holds that
% 
\begin{align*}
    1 = \sum_{i,j\in[n]} \left[f(M^* + E_{ij}; M^*) - f(M^*;M^*) \right] \leq \frac{c_2}{2} \cdot \sum_{i,j\in[n]} \|E_{ij}\|_F^2 = \frac{c_2 n^2}{2},
\end{align*}
% 
which implies that $c_2 \geq 2 n^{-2}$. Using the relation $c_2/c_1 = (1+\delta)/(1-\delta)$, we obtain that
% 
\[ c_1 \geq \frac{2(1-\delta)}{n^2(1+\delta)}. \]
% 
By substituting into inequality \eqref{eqn:rip-general-1}, it follows that
% 
\[ \|f(\cdot;M^*) - \tilde{f}(\cdot;\tilde{M}^*)\|_1 \geq \frac{1-\delta}{n^2(1+\delta)}. \]
% 
which leads to $\dist_\alpha[ (f,M^*), (\tilde{f},\tilde{M}^*) ] \geq \alpha(1-\delta)/[n^2(1+\delta)]$. Now, the desired bound on $\mathbb{D}_\alpha(f,M^*)$ follows from taking the inverse. In the case when $M = M^*$, we can replace $M$ with $\tilde{M}^*$ and the proof can be done in the same way.
\qed\end{proof}

We note that in Theorems \ref{thm:rip-1} and \ref{thm:rip-gen}, the normalization constraint on $u^*$ is not used. Therefore, the upper bound may be loose for certain instances since the information about the global solution is not used. 


